On the Theoretical Limits of Beam Steering in mmWave Massive MIMO Channels

Analog Beamsteering (ABS) has emerged as a low complexity, power efficient solution for MillimeterWave (mmWave) massive Multiple Input Multiple Output (MIMO) systems. Moreover, driven by the low spatial correlation between the User Terminals (UTs) with high number of transmit antennas (massive MIMO) at the Base Station (BS), ABS can be used to support Multi User (MU) MIMO scenarios instead of digital or Hybrid Beamforming (HBF). However, we show in this paper, that even with high number of transmit antennas, the HBF can achieve better Spectral Efficiency (SE) compared to the MU ABS even in pure Line of Sight (LoS) channels. Moreover, we prove that the MU ABS saturates to a constant SE at high transmit Signal to Noise Ratio (SNR) and we theoretically derive an approximation to that saturation bound in this paper. On the other hand, we highlight that the HBF's SE scales with the transmit SNR even in high SNR regime. Finally, given the same power consumption and hardware complexity as the MU ABS case, we show that HBF asymptotically achieves the optimal SE (ideal non interference scenario) when increasing the number of transmit antennas.

==> sections/1_introduction.tex <==
Here goes the introduction
